Phoebus: Performance Portable GRRMHD for Relativistic Astrophysics

We introduce the open source code PHOEBUS (phifty one ergs blows up a star) for astrophysical general relativistic radiation magnetohydrodynamic simulations. PHOEBUS is designed for, but not limited to, high energy astrophysical environments such as core-collapse supernovae, neutron star mergers, black-hole accretion disks, and similar phenomena. General relativistic magnetohydrodynamics are modeled in the Valencia formulation with conservative finite volume methods. Neutrino radiation transport is included with Monte Carlo and moment methods. PHOEBUS is built on the PARTHENON (Grete et al. 2022) performance portable adaptive mesh refinement framework, uses a GPU first development strategy, and is capable of modeling a large dynamic range in space and time. PHOEBUS utilizes KOKKOS for on-node parallelism and supports both CPU and GPU architectures. We describe the physical model employed in PHOEBUS, the numerical methods used, and demonstrate a suite of test problems to showcase its abilities. We demonstrate weak scaling to over 500 H100 GPUs.

==> journal_abbr.tex <==
\newcommand\aj{AJ}% 
          % Astronomical Journal 
\newcommand\araa{ARA\&A}% 
          % Annual Review of Astron and Astrophys 
\newcommand\apj{ApJ}% 
          % Astrophysical Journal 
\newcommand\apjl{ApJ}% 
          % Astrophysical Journal, Letters 
\newcommand\apjs{ApJS}% 
          % Astrophysical Journal, Supplement 
\newcommand\ao{Appl.~Opt.}% 
          % Applied Optics 
\newcommand\apss{Ap\&SS}% 
          % Astrophysics and Space Science 
\newcommand\aap{A\&A}% 
          % Astronomy and Astrophysics 
\newcommand\aapr{A\&A~Rev.}% 
          % Astronomy and Astrophysics Reviews 
\newcommand\aaps{A\&AS}% 
          % Astronomy and Astrophysics, Supplement 
\newcommand\azh{AZh}% 
          % Astronomicheskii Zhurnal 
\newcommand\baas{BAAS}% 
          % Bulletin of the AAS 
\newcommand\jrasc{JRASC}% 
          % Journal of the RAS of Canada 
\newcommand\memras{MmRAS}% 
          % Memoirs of the RAS 
\newcommand\mnras{MNRAS}% 
          % Monthly Notices of the RAS 
\newcommand\pra{Phys.~Rev.~A}% 
          % Physical Review A: General Physics 
\newcommand\prb{Phys.~Rev.~B}% 
          % Physical Review B: Solid State 
\newcommand\prc{Phys.~Rev.~C}% 
          % Physical Review C 
\newcommand\prd{Phys.~Rev.~D}% 
          % Physical Review D 
\newcommand\pre{Phys.~Rev.~E}% 
          % Physical Review E 
\newcommand\prl{Phys.~Rev.~Lett.}% 
          % Physical Review Letters 
\newcommand\pasp{PASP}% 
          % Publications of the ASP 
\newcommand\pasj{PASJ}% 
          % Publications of the ASJ 
\newcommand\qjras{QJRAS}% 
          % Quarterly Journal of the RAS 
\newcommand\skytel{S\&T}% 
          % Sky and Telescope 
\newcommand\solphys{Sol.~Phys.}% 
          % Solar Physics 
\newcommand\sovast{Soviet~Ast.}% 
          % Soviet Astronomy 
\newcommand\ssr{Space~Sci.~Rev.}% 
          % Space Science Reviews 
\newcommand\zap{ZAp}% 
          % Zeitschrift fuer Astrophysik 
\newcommand\nat{Nature}% 
          % Nature 
\newcommand\iaucirc{IAU~Circ.}% 
          % IAU Cirulars 
\newcommand\aplett{Astrophys.~Lett.}% 
          % Astrophysics Letters 
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}% 
          % Astrophysics Space Physics Research 
\newcommand\bain{Bull.~Astron.~Inst.~Netherlands}% 
          % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{Fund.~Cosmic~Phys.}% 
          % Fundamental Cosmic Physics 
\newcommand\gca{Geochim.~Cosmochim.~Acta}% 
          % Geochimica Cosmochimica Acta 
\newcommand\grl{Geophys.~Res.~Lett.}% 
          % Geophysics Research Letters 
\newcommand\jcp{J.~Chem.~Phys.}% 
          % Journal of Chemical Physics 
\newcommand\jgr{J.~Geophys.~Res.}% 
          % Journal of Geophysics Research 
\newcommand\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}% 
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{Mem.~Soc.~Astron.~Italiana}% 
          % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{Nucl.~Phys.~A}% 
          % Nuclear Physics A 
\newcommand\physrep{Phys.~Rep.}% 
          % Physics Reports 
\newcommand\physscr{Phys.~Scr}% 
          % Physica Scripta 
\newcommand\planss{Planet.~Space~Sci.}% 
          % Planetary Space Science 
\newcommand\procspie{Proc.~SPIE}% 
          % Proceedings of the SPIE 
\newcommand\jcphys{J.~Comp.~Phys.}% 
          % Journal of Computational Physics

\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 

